Bayesian Optimization for Probabilistic Programs

We present the first general purpose framework for marginal maximum a posteriori estimation of probabilistic program variables. By using a series of code transformations, the evidence of any probabilistic program, and therefore of any graphical model, can be optimized with respect to an arbitrary subset of its sampled variables. To carry out this optimization, we develop the first Bayesian optimization package to directly exploit the source code of its target, leading to innovations in problem-independent hyperpriors, unbounded optimization, and implicit constraint satisfaction; delivering significant performance improvements over prominent existing packages. We present applications of our method to a number of tasks including engineering design and parameter optimization.

==> optquery.tex <==
% !TEX root =  bopp.tex

%In this section we introduce a set of requirements for an ``optimization query", which returns an infinite lazy sequence of increasingly optimal estimates for some target variables $\theta \in \vartheta$.  For exposition purposes, we first consider the case where $\theta$ correspond to the inputs of a query $q$ and show how this can be extended to arbitrary variables within the program in section \ref{sec:transform}. We assume $q$ takes as inputs, along with $\theta$ data upon which the query is conditioned $Y$.


%As it is only possible to estimate $p(Y, \hth_m)$ such that
%\begin{align}
%\label{eq:BOPPoutput}
%E_f\left[\hat{p} \left(Y,\hth_m\right) | D_{m} \right] \ge E_f\left[\hat{p} \left(Y,\hth_j\right) | D_{m} \right] \quad \forall j=1,\dots,m-1
%\end{align}
%where $\hat{p}$ is used to indicate that the estimation of the marginal probability is itself probabilistic due to the approximation nature of inference. 

Given the above program transformation we can use a generic inference method provided by the back end to marginalize over the latent variables $X$ conditioned on $\theta$. We will here use sequential Monte Carlo for probablistic programs \citep{wood2014new} to obtain unnormalized estimates of the marginal conditional likelihood
\begin{align}
\hw \left(Y,\theta\right) \approx p\left(Y | \theta\right) =\int p\left(X,Y|\theta\right) dX.
\end{align}
Given these estimates we are now in a position to define the problem setting for MMAP estimation in probabilistic programs. Specifically we will define a macro \lsi{doopt} that accept a query defined using \lsi{defopt} and returns a lazy sequence of increasingly optimal estimates for the target variables $\theta$. We now formally define our optimization query to output an infinite lazy sequence $\{\hth_1,\hat{\Omega}_1\},\{\hth_2,\hat{\Omega}_2\},\dots$ where $\hat{\Omega}_i$ is the map of \predict values with the query when $\theta=\hth_i$ and
\begin{align}
\label{eq:BOPPoutput}
E\left[\hw \left(Y,\hth_m\right) p\left(\hth_m\right) | D_{m} \right] \ge E\left[\hw \left(Y,\hth_j\right) p\left(\hth_j\right) | D_{m} \right] \quad \forall j=1,\dots,m-1 \quad m=1,2,\dots
\end{align}
where the expectation is over the surrogate function posterior. $\hth_m$ corresponds to the point that is expected to be the most optimal of those evaluated under the posterior of our surrogate function. Since evaluations of are noisy, this need not be the $\theta$ value that produced the highest the $p(\theta)$-weighted marginal likelihood estimate. % Further as the observation of a new point affects the surrogate function posterior at all other points (as the expectation of both sides of~\eqref{eq:BOPPoutput} is conditioned on all data observed so far $D_m$), $\hth_m$ can change between different historical values when a new point is queried.


% Consider a generic query $q$.  Let the \sample statements within the $q$ define a generative distribution for a set of latent variables $X = \left\{x_{i}\right\}_{i=1,\dots,N}, \; X \in \mathcal{X}$ (note $x_i$ may have different support for different $i$) with prior $p\left(X | \theta\right) = p\left(x_1 | \theta\right) \prod_{i=2}^{N} p\left(x_i | x_1,\dots,x_{i-1},\theta\right)$, parametrized by a set of program inputs $\theta \in \vartheta$.  Let the \observe statements in the program define conditioning on observations $Y = \left\{y_i\right\}_{i=1,\dots,N}, \; Y \in \mathcal{Y}$ such that the query defines the joint factorization\footnote{Note, there is notational deficiency as in a higher-order PPS variable types, the order of the conditioning for the latent variables and even the number of latent variables can change depending on the program trace.}
% \begin{multline}
% \label{eq:Joint}
% p\left(X,Y|\theta\right) = p\left(x_1 | \theta\right) p\left(y_1 | x_1, \theta\right) \\ \prod_{i=2}^{N} p\left(y_i | x_1,\dots,x_{i},\theta\right) p\left(x_i | x_1,\dots,x_{i-1},\theta\right).
% \end{multline}
% We assume that the observations $Y$ are fixed and finite dimensional.  Our aim is to optimize the marginal likelihood of this joint scaled by a prior on $\theta$:
% \begin{align}
% \label{eq:hyperOpt}
% \theta^* = \argmax_{\theta \in \vartheta} p\left(\theta\right) \int_{X}^{} p\left(X,Y|\theta\right) dX,
% \end{align}

%Often the prior on $\theta$ will often correspond only to a set of bounds, giving a uniform distribution within the permissible input space.  If $p\left(\theta\right)$ is allowed to be potentially improper,~\eqref{eq:hyperOpt} also incorporates maximum likelihood estimation .  
%restricting the choice of inference algorithm. Anglican supports a number of suitable algorithms including importance sampling \citep{glynn1989importance}, sequential Monte Carlo (SMC) \citep{smith2013sequential,wood_aistats_2014} and the particle cascade \citep{paige2014asynchronous}.


For clarity we introduce the following notation of the rest of the paper.  We use $\theta_m$ to refer to the $\theta$ used to call the query at iteration $m$, and $\Omega_m$ and $W_m$ for the predicts and marginal likelihood estimate from this call respectively.  We define $\jsm \in \{1,\dots,m\}$ to be the index corresponding to the estimated best $\theta_m$ at iteration $m$ such that $\hth_m = \theta_{\jsm}$.  We further define $Z_m \coloneqq W (Y,\theta_j) p(\theta_j)$ and $\hz_m \coloneqq \hw (Y,\hth_j) p(\hth_j)$ as the corresponding estimates of the weighted marginal weights.

%We finally note that our optimization query includes as a special case independent calls to an inference query by setting $\ell (\cdot) = 0$ and by convention taking the most recent sample under equality of~\eqref{eq:BOPPoutput}.  Furthermore, one is free to choose the sequence of $\tilth$ in anyway desired.  For example, one may wish to explicitly control the trade off between improving our estimates for $\theta^*$, and refining the inference of the latent variables $p(z | y, \tilth_{\jsm})$ by recalling the original query with the same $\theta$.

